AugLift: Depth-Aware Input Reparameterization Improves Domain Generalization in 2D-to-3D Pose Lifting

Lifting-based 3D human pose estimation infers 3D joints from 2D keypoints but generalizes poorly because $(x,y)$ coordinates alone are an ill-posed, sparse representation that discards geometric information modern foundation models can recover. We propose \emph{AugLift}, which changes the representation format of lifting from 2D coordinates to a 6D geometric descriptor via two modules: (1) an \emph{Uncertainty-Aware Depth Descriptor} (UADD) -- a compact tuple $(c, d, d_{\min}, d_{\max})$ extracted from a confidence-scaled neighborhood of an off-the-shelf monocular depth map -- and (2) a scale normalization component that handles train/test distance shifts. AugLift requires no new sensors, no new data collection, and no architectural changes beyond widening the input layer; because it operates at the representation level, it is composable with any lifting architecture or domain generalization technique. In the detection setting, AugLift reduces cross-dataset MPJPE by $10.1$% on average across four datasets and four lifting architectures while improving in-distribution accuracy by $4.0$%; post-hoc analysis shows gains concentrate on novel poses and occluded joints. In the ground-truth 2D setting, combining AugLift with PoseAug's differentiable domain generalization achieves state-of-the-art cross-dataset performance ($62.4$\,mm on 3DHP, $92.6$\,mm on 3DPW; $14.5$% and $22.2$% over PoseAug), demonstrating that foundation-model depth provides genuine geometric signal complementary to explicit 3D augmentation. Code will be made publicly available.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec/0_abstract_tmp.tex <==
\begin{abstract}
Lifting-based 3D human pose estimators infer 3D joints from 2D keypoints, but often struggle to generalize to real-world settings that rely on noisy 2D detections. We revisit the \emph{input} to lifting and propose \emph{AugLift}, a simple augmentation of standard lifting that enriches each 2D keypoint $(x,y)$ with an Uncertainty-Aware Depth Descriptor (UADD). We first run a single off-the-shelf monocular depth estimator on the image to obtain a depth map, and for every keypoint with detector confidence $c$ we extract depth statistics from its confidence-scaled neighborhood, forming a compact, interpretable UADD $(c, d, d_{\min}, d_{\max})$ that captures both local geometry and reliability. AugLift is modular---it requires no new sensors, data collection, or architectural changes—and integrates by expanding the input layer of existing lifting models.

Across four datasets and four lifting architectures, AugLift boosts cross-dataset (out-of-distribution, OOD) performance on unseen datasets by an average of $10.1\%$, while also improving in-distribution (ID) performance by $4.0\%$, as measured by MPJPE. A post-hoc analysis clarifies \emph{when} and \emph{why} it helps: gains are largest on novel poses and significantly occluded joints, where depth statistics resolve front--back ambiguities while confidence calibrates the spatial neighborhoods from which they are drawn. Finally, we study interaction with recent image-feature lifting methods and find the signals are complementary: adding UADD to image-conditioned lifting yields both ID and OOD gains. Moreover, a learned depth-feature extension (AugLiftV2) improves performance further while trading off interpretability. Together, these results indicate that lightweight, confidence-aware depth cues are a powerful plug-in for robust 2D--3D pose lifting. 
Code will be made publicly available.
\keywords{3D Human Pose Estimation \and Domain Generalization \and Monocular Depth \and Uncertainty}
\end{abstract}

% \begin{abstract}
% Lifting-based 3D human pose estimators infer 3D joints from 2D keypoints, but often struggle to generalize to real-world settings that rely on noisy 2D detections. We revisit the \emph{input} to lifting and propose \emph{AugLift}, a simple augmentation of standard lifting that enriches each 2D keypoint $(x,y)$ with an Uncertainty-Aware Depth Descriptor (UADD). We first run a single off-the-shelf monocular depth estimator on the image to obtain a depth map, and for every keypoint with detector confidence $c$ we extract depth statistics from its confidence-scaled neighborhood, forming a compact, interpretable UADD $(c, d, d_{\min}, d_{\max})$ that captures both local geometry and reliability. AugLift is modular---it requires no new sensors, data collection, or architectural changes---and integrates by expanding the input layer of existing lifting models.

% Across four datasets and four lifting architectures, AugLift boosts cross-dataset (out-of-distribution, OOD) performance on unseen datasets by an average of $10.1\%$, while also improving in-distribution (ID) performance by $4.0\%$, as measured by MPJPE. A post-hoc analysis clarifies \emph{when} and \emph{why} it helps: gains are largest on \emph{novel} poses and \emph{moderately to heavily occluded} joints, where depth statistics resolve front--back ambiguities while confidence calibrates the spatial neighborhoods from which they are drawn. Finally, we study interaction with recent image-feature lifting methods and find the signals are complementary: adding UADD to image-conditioned lifting yields both ID and OOD gains, and a learned depth-feature extension (AugLiftV2) improves performance further while trading off interpretability. Together, these results indicate that lightweight, confidence-aware depth cues are a powerful plug-in for robust 2D--3D pose lifting.
% \end{abstract}



% \begin{abstract}
% Lifting‑based 3D human pose estimators infer 3D joints from 2D keypoints, but often struggle to generalize to real-world settings that rely on noisy 2D detections. We revisit the \emph{input} to lifting and propose \emph{AugLift}, a simple augmentation of standard lifting that enriches each 2D joint $(x,y)$ with an Uncertainty‑Aware Depth Descriptor (UADD). For every keypoint with detector confidence $c$, we run a monocular depth estimator and extract depth statistics from a confidence‑scaled neighborhood, yielding a compact, interpretable vector $(c, d, d_{\min}, d_{\max})$ that captures both geometric context and reliability. AugLift is modular—no new sensors or architectural changes—and integrates by expanding the input layer.

% Across datasets and backbones, AugLift improves in‑distribution (ID) performance and, more notably, OOD generalization (e.g., average MPJPE reductions of $10.1\%$ OOD and $4.0\%$ ID in our cross‑dataset study), at modest overhead from the depth pass. A post‑hoc analysis clarifies \emph{when} and \emph{why} it helps: gains are largest on \emph{novel} poses and \emph{moderately/heavily occluded} joints, where depth statistics resolve front–back ambiguities while confidence calibrates spatial neighborhoods. Finally, we study interaction with recent image‑feature lifting methods and find the signals are complementary; adding UADD to image‑conditioned lifting yields further gains, and a learned depth‑feature extension (AugLiftV2) improves performance further while trading off interpretability. Together, these results indicate that lightweight, confidence‑aware depth cues are a powerful plug‑in for robust 2D–3D pose lifting.
% \end{abstract}


% \begin{abstract}
% We propose \textbf{AugLift}, a \emph{simple augmentation} of standard 2D–3D pose lifting that concatenates an \emph{uncertainty‑aware depth descriptor} (UADD) to each 2D joint. For a keypoint with confidence $c$, UADD aggregates monocular‑depth statistics $(d, d_{\min}, d_{\max})$ from a confidence‑scaled neighborhood, yielding an interpretable vector $(c, d, d_{\min}, d_{\max})$ that provides geometric context and reliability cues. AugLift is modular (no new sensors or architectural changes) and consistently improves both ID accuracy and OOD generalization across datasets/backbones (e.g., average MPJPE reductions of $10.1\%$ OOD and $4.0\%$ ID), with modest additional cost for the depth pass. Post‑hoc analysis shows AugLift helps most on \emph{novel} and \emph{occluded} poses by resolving depth ambiguities when 2D is reliable and by supplying lower‑bound depth cues under occlusion. AugLift is complementary to image‑feature‑conditioned lifting, and a learned depth‑feature extension (AugLiftV2) further improves performance while trading interpretability.
% \end{abstract}

==> sec/1_intro_tmp.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.5\textwidth]{figures/auglift_fig1_v2.png}
\vspace{-10pt}
\caption{\textbf{AugLift Enriches Standard Lifting Inputs for Better Generalization.}
Standard lifting models use only sparse 2D coordinates (x,y), which creates ambiguity. Conditioning on dense image or depth maps tends to overfit to domain-specific backgrounds and appearance. AugLift instead enriches—rather than replaces—the (x,y) input using two signals: a monocular depth map and keypoint confidence. Local depth statistics (d, d\textsubscript{min}, d\textsubscript{max}) combined with confidence (c) form a compact Uncertainty-Aware Depth Descriptor (UADD), which delivers high-quality geometric cues that generalize well to cases with occlusion or novel poses.}
\label{fig:system_diagram}
\vspace{-10pt}
\end{figure}

Estimating 3D human pose from monocular RGB is a long-standing problem in computer vision, with applications in graphics, robotics, AR/VR, and sports analysis.
A widely adopted paradigm decomposes the task into two stages: a 2D keypoint detector first localizes joints in the image, and a \emph{lifting} model then maps these 2D keypoints to 3D joint locations~\cite{martinez2017simple, pavllo2018video, zhu2023motionbert}.
This two-stage approach leverages strong 2D pose estimators and cleanly separates perception from geometry.
However, lifting-based 3D human pose estimators often struggle to generalize beyond the lab-style conditions of their training sets, especially in realistic \emph{detection settings} where they must consume noisy 2D keypoints instead of ground-truth annotations.

There are two main reasons for this generalization gap.
First, 2D keypoints are an extremely \emph{sparse} representation of the image: by design they discard most geometric and appearance information that could help disambiguate depth, occlusion, and viewpoint.
Second, in practice, lifting models are typically trained on curated datasets with limited diversity in camera setups, backgrounds, and motion patterns.
As a result, they tend to overfit to the idiosyncrasies of the training distribution, making them brittle to  cross-dataset transfer even when the underlying 2D detector is reasonably robust.
Recent benchmarks show that state-of-the-art lifting networks achieving $40$--$50$mm MPJPE on Human3.6M can degrade to over $100$mm on in-the-wild datasets such as 3DPW when using detected 2D keypoints~\cite{manzur2025posebench3d, wang2020predicting}. We visualize the difficulty of out of distribution generalization in Appendix Figure \ref{fig:generalization_gap}. 



A natural way to address this limitation is to enrich the lifting input. Some methods leverage temporal context from video sequences~\cite{pavllo2018video, zhu2023motionbert}, while others attempt to condition the lifting model on image features~\cite{xu2022monocular, zhou2023lifting}. However, these approaches often struggle to generalize. For example, learned priors may focus more on background pixels than the subject itself~\cite{zhou2023lifting}, and the use of temporal context makes generalization to novel actions challenging.
% \niko{Add reference to old figure 2 of generalization error here.}
% A natural way to address this limitation is to enrich the lifting input with additional cues that provide geometric context while remaining compatible with the two-stage pipeline.
% Recent works have explored incorporating image features or depth information into lifting, either by conditioning on CNN feature maps or by introducing auxiliary depth supervision~\cite{nie2019view,zhou2024lifting_by_image,jiang2021ordinaldepth}.
% While promising, these approaches often require heavier architectures, careful feature-fusion design, or additional annotations.
In parallel, modern monocular depth estimators have made striking progress and generalize well across scenes and datasets, yet their potential as a plug-in signal for 2D--3D lifting remains underexplored.

In this work we revisit the \emph{input} to lifting and ask:
can we improve robustness and generalization simply by augmenting the 2D keypoints with lightweight depth cues?
To this end, we propose \emph{AugLift}, a simple augmentation of standard lifting that enriches each 2D keypoint $(x,y)$ with an \emph{Uncertainty-Aware Depth Descriptor} (UADD).
Concretely, we first run a single off-the-shelf monocular depth estimator on the input image to obtain a depth map.
For every keypoint with detector confidence $c$, we extract summary depth statistics from a \emph{confidence-scaled neighborhood} around the keypoint, forming a compact, interpretable UADD $(c, d, d_{\min}, d_{\max})$ that captures both local geometry and reliability.
AugLift is modular---it requires no new sensors, data collection, or architectural changes---and integrates into existing lifters by simply expanding the input layer from $2K$ to $6K$ channels (for $K$ joints).

We validate AugLift through a series of comprehensive experiments.
Across four diverse datasets and four different lifting architectures in the detection setting, AugLift consistently and significantly improves performance in both cross-dataset (out-of-distribution, OOD) and within-dataset (in-distribution, ID) scenarios.
For instance, when integrated with a state-of-the-art model (MotionBERT~\cite{zhu2023motionbert}), AugLift boosts cross-dataset performance by an average of $10.1\%$ while simultaneously improving in-distribution performance by $4.0\%$, as measured by the reduction in MPJPE.

Beyond proposing this augmentation, we seek to understand \emph{when and why} such depth cues help.
Our analysis reveals that AugLift is particularly effective on \emph{novel} poses not seen at training and on \emph{moderately to heavily occluded} joints.
In these regimes, the depth statistics help resolve front--back ambiguities (for novel poses) and provide robust lower-bound cues on joint depth (for occlusion), while the confidence signal regulates how aggressively the neighborhood should be expanded.
We also study how AugLift complements recent lifting methods that fuse RGB image features. Finally, we introduce an extension that replaces the handcrafted UADD with learned depth-image features, trading interpretability for additional gains.
 
\begin{figure}[tb]
    \centering

    % Row 1
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/5_2c.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/5_3c.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/depth_estimate_fig4.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/UADD_fig4_v2.png}
    \end{minipage}
    
    % Row 2
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/5_2d.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/5_3d.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/keypoint_conf_fig4_v3.png}
    \end{minipage}
    \begin{minipage}{0.16\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=\linewidth]{figures/depth_variability_fig4_v2.png}
    \end{minipage}
    

    \vspace{-6pt}
    \caption{\textbf{How AugLift Learns to Trust Keypoints via Adaptive Uncertainty Sampling. }  \textbf{Left}:  We visualize the two signals that augment the standard lifting input: 2D keypoint confidence (top) and a monocular depth map (bottom). Confidence scores act as a proxy for visibility (blue = confident, red X = unconfident), while the depth map captures the 3D structure (blue = near, red = far).
    \textbf{Right}: AugLift implements confidence-aware sampling by using the confidence score to define a sampling radius that is inversely proportional to it. As shown, low-confidence (often occluded) joints use a wider sampling radius to gather robust depth statistics while high-confidence joints use a small, localized radius for a precise estimate. This allows the model to learn to identify and distrust unreliable depth estimates.
    % \niko{todo: cleanup up right graphics, placeholder}
    }
    \label{fig:depth_confidence}
\end{figure}

\vspace{-5pt}

% Visualization of confidence-aware depth sampling. 
%     The 2D keypoint confidence is used to define a sampling cone inversely proportional to confidence—lower-confidence keypoints correspond to wider regions. 
%     Within this region, we sample depth statistics such as the minimum, maximum, and the pointwise depth at the detected 2D location. 
%     These statistics are concatenated into a feature vector representing the local geometric uncertainty, which is fed into the lifting network. 
%     This enables the model to learn when depth estimates are reliable versus unreliable.
%     \niko{Replace with higher resolution, only first 2 rows.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/depth_uncertainty.png}
%     \caption{Visualization of confidence-aware depth sampling. 
%     The 2D keypoint confidence is used to define a sampling cone inversely proportional to confidence—lower-confidence keypoints correspond to wider regions. 
%     Within this region, we sample depth statistics such as the minimum, maximum, and the pointwise depth at the detected 2D location. 
%     These statistics are concatenated into a feature vector representing the local geometric uncertainty, which is fed into the lifting network. 
%     This enables the model to learn when depth estimates are reliable versus unreliable.
%     \niko{Replace with higher resolution, only first 2 rows.}}
%     \label{fig:depth_uncertainty}
% \end{figure}



\noindent\textbf{Contributions.}
Our main contributions are as follows:
\begin{itemize}
    \item \textbf{C1.}
    We propose \emph{AugLift}, a simple, modular augmentation of standard 2D--3D lifting that enriches each 2D keypoint with an Uncertainty-Aware Depth Descriptor (UADD) computed from an off-the-shelf monocular depth estimator, yielding a 6D per-joint input that can be plugged into existing lifting architectures without changing their core design.
    % We propose \emph{AugLift}, a simple, modular augmentation of standard 2D--3D lifting that enriches each 2D keypoint with an uncertainty-aware depth descriptor computed from an off-the-shelf monocular depth estimator and keypoint confidence score.
    % UADD combines detector confidence with summary statistics of local depth in a confidence-scaled neighborhood, and can be plugged into existing lifting architectures without altering their core design.

    \item \textbf{C2.}
    We conduct a systematic study across four datasets and four lifting architectures, focusing on the critical intersection of cross-dataset (OOD) generalization and the realistic 2D detections setting. In this challenging regime, AugLift consistently improves performance, yielding average MPJPE reductions of 10.1\% OOD and 4.0\% ID.
    % We conduct a systematic study across four datasets and four lifting architectures, focusing on the critical, yet understudied, intersection of cross-dataset (OOD) generalization and the realistic 2D detections setting. In this challenging domain, AugLift consistently improves performance, yielding average MPJPE reductions of 10.1\% OOD and 4.0\% ID.
    % We conduct a systematic empirical study across four datasets and four lifting architectures in the realistic detection setting.
    % AugLift consistently improves both in-distribution (ID) accuracy and, more prominently, cross-dataset (out-of-distribution, OOD) performance, yielding average MPJPE reductions of 10.1\% OOD and 4.0\%, while incurring only modest additional cost from the depth pass.

    \item \textbf{C3.}
    We provide a detailed post-hoc analysis explaining when and why AugLift works. We show that the largest gains occur on the most challenging cases: novel poses not seen during training (e.g., a 15.7\% error reduction on Fit3D) and significantly occluded joints.
    % We provide a detailed post-hoc analysis explaining when and why AugLift works. We show that the largest gains occur on the most challenging cases: novel poses not seen during training (e.g., a 15.7\% error reduction on Fit3D) and significantly occluded joints.
    % We provide a detailed post-hoc analysis explaining when and why AugLift works. 
    % We demonstrate that the largest performance gains are on the most challenging cases: novel poses not seen during training (e.g., -15.7\% error on Fit3D) and significantly occluded joints.
    
    % Gains are largest on occluded and dissimilar poses; for instance, the median error reduction on Fit3D more than doubles for the most occluded quartile of frames (9.4\%) compared to the clearest (4.1\%)

    \item \textbf{C4.} 
    We demonstrate that AugLift's sparse geometric cues are complementary to dense image features, with their combination achieving the strongest out-of-distribution (OOD) improvement of 10.5\%. We also introduce AugLiftV2, a \textit{learned} extension that trades interpretability for even larger gains.
    % We demonstrate that AugLift's sparse geometric cues are complementary to dense image features, with their combination achieving the strongest out-of-distribution (OOD) improvement of 10.5\%. We also introduce AugLiftV2, a learned extension that trades interpretability for even larger in-distribution (ID) gains of 11.8\% and opens a new avenue for depth-feature fusion.
    % We show AugLift’s sparse cues are complementary to dense image features. In a pilot study with PoseFormer, a learned depth-feature extension (AugLiftV2) combined with image feature fusion improves in-distribution performance by 11.8\% and out-of-distribution performance by 9.1\% relative to the baseline.

    
    
    
    
    
    
    
    
    % \item \textbf{C3.} We provide a deeper analysis of \emph{when} and \emph{why} AugLift helps.
    % Our clustering analysis reveals that AugLift gains are largest on novel poses and significantly occluded joints through the synergistic use of confidence and depth cues.I
    % We find that lifting with AugLift and by fusing image features are complementary and thus optimal to combine. Finally, a learned depth-feature extension (AugLiftV2) improves performance further while trading off interpretability.
    
    % \niko{Should we put quantiative statistics here (~11.8\% indistr, ~9.1\% ood}

    % \item \textbf{C3.} We provide a post-hoc analysis of \emph{when} and \emph{why} AugLift helps.
    % By clustering poses according to their novelty relative to the training set and stratifying joints by occlusion level, we show that gains are largest on novel poses and significantly occluded joints, and we illustrate how confidence and depth cues interact to resolve depth ambiguities.
    % We further study the interaction between AugLift and image-feature-conditioned lifting, showing that the signals are complementary, and we explore a learned depth-feature extension (AugLiftV2) that improves performance further while trading off interpretability.
\end{itemize}

% \noindent
% The remainder of the paper is organized as follows.
% Section~\ref{sec:lit_review} reviews related work in lifting-based 3D human pose estimation, monocular depth, and feature-fusion approaches.
% Section~\ref{sec:methods} describes the standard lifting setup and introduces AugLift and UADD in detail.
% Section~\ref{sec:experiments} presents our experimental setup and core results across datasets and architectures.
% Section~\ref{sec:analysis} analyzes when and why AugLift helps, including its interaction with image features and the AugLiftV2 extension that uses learned depth features.
% Finally, Section~\ref{sec:conclusion} discusses limitations and concludes.





% \section{Introduction}
% \label{sec:intro}

% Estimating 3D human pose from monocular RGB is a long-standing problem in computer vision, with applications in graphics, robotics, AR/VR, and sports analysis.
% A widely adopted paradigm decomposes the task into two stages: a 2D keypoint detector first localizes joints in the image, and a \emph{lifting} model then maps these 2D keypoints to 3D joint locations.
% This two-stage approach leverages strong 2D pose estimators and cleanly separates perception from geometry.
% However, lifting-based 3D human pose estimators often struggle to generalize beyond the lab-style conditions of their training sets, especially in realistic \emph{detection settings} where they must consume noisy 2D keypoints instead of ground-truth annotations.

% There are two main reasons for this generalization gap.
% First, 2D keypoints are an extremely \emph{sparse} representation of the image: by design they discard most geometric and appearance information that could help disambiguate depth, occlusion, and viewpoint.
% Second, in practice, lifting models are typically trained on curated datasets with limited diversity in camera setups, backgrounds, and motion patterns.
% As a result, they tend to overfit to the idiosyncrasies of the training distribution:
% they are brittle to occlusions and self-occlusions, they confuse front--back ambiguous poses, and they degrade significantly under cross-dataset transfer, even when the underlying 2D detector is reasonably robust.

% A natural way to address this limitation is to enrich the lifting input with additional cues that provide geometric context while remaining compatible with the two-stage pipeline.
% Recent works have explored incorporating image features or depth information into lifting, but these approaches often require heavier architectures, careful feature-fusion design, or additional supervision.
% In parallel, modern monocular depth estimators have made striking progress and generalize well across scenes and datasets, yet their potential as a plug-in signal for 2D--3D lifting remains underexplored.

% In this work we revisit the \emph{input} to lifting and ask:
% can we improve robustness and generalization simply by augmenting the 2D keypoints with lightweight depth cues?
% To this end, we propose \emph{AugLift}, a simple augmentation of standard lifting that enriches each 2D keypoint $(x,y)$ with an \emph{Uncertainty-Aware Depth Descriptor} (UADD).
% Concretely, we first run a single off-the-shelf monocular depth estimator on the input image to obtain a depth map.
% For every keypoint with detector confidence $c$, we extract summary depth statistics from a \emph{confidence-scaled neighborhood} around the keypoint, forming a compact, interpretable UADD $(c, d, d_{\min}, d_{\max})$ that captures both local geometry and reliability.
% AugLift is modular---it requires no new sensors, data collection, or architectural changes---and integrates into existing lifters by simply expanding the input layer from $2K$ to $6K$ channels (for $K$ joints).

% Beyond proposing this augmentation, we seek to understand \emph{when and why} such depth cues help.
% Our analysis reveals that AugLift is particularly effective on \emph{novel} poses that differ from the training motion patterns and on \emph{moderately to heavily occluded} joints.
% In these regimes, the depth statistics help resolve front--back ambiguities (for novel poses) and provide robust lower-bound cues on joint depth (for occlusion), while the confidence signal regulates how aggressively the neighborhood should be expanded.
% We also study how AugLift complements recent lifting methods that fuse RGB image features, and we introduce an extension that replaces the handcrafted UADD with learned depth-image features, trading interpretability for additional gains.

% \paragraph{Contributions.}
% Our main contributions are as follows:
% \begin{itemize}
%     \item \textbf{C1.} We propose \emph{AugLift}, a simple, modular augmentation of standard 2D--3D lifting that enriches each 2D keypoint with an \emph{uncertainty-aware depth descriptor} (UADD) computed from an off-the-shelf monocular depth estimator.
%     UADD combines detector confidence with summary statistics of local depth in a confidence-scaled neighborhood, and can be plugged into existing lifting architectures without altering their core design.

%     \item \textbf{C2.} We conduct a systematic empirical study across four datasets and four lifting architectures in the realistic detection setting.
%     AugLift consistently improves both in-distribution (ID) accuracy and, more prominently, cross-dataset (out-of-distribution, OOD) performance, yielding average MPJPE reductions of $10.1\%$ OOD and $4.0\%$ ID, while incurring only modest additional cost from the depth pass.

%     \item \textbf{C3.} We provide a post-hoc analysis of \emph{when} and \emph{why} AugLift helps.
%     By clustering poses according to their novelty relative to the training set and stratifying joints by occlusion level, we show that gains are largest on novel poses and significantly occluded joints, and we illustrate how confidence and depth cues interact to resolve depth ambiguities.
%     We further study the interaction between AugLift and image-feature-conditioned lifting, showing that the signals are complementary, and we explore a learned depth-feature extension (AugLiftV2) that improves performance further while trading off interpretability.
% \end{itemize}

% \noindent
% The remainder of the paper is organized as follows.
% Section~\ref{sec:lit_review} reviews related work in lifting-based 3D human pose estimation, monocular depth, and feature-fusion approaches.
% Section~\ref{sec:methods} describes the standard lifting setup and introduces AugLift and UADD in detail.
% Section~\ref{sec:experiments} presents our experimental setup and core results across datasets and architectures.
% Section~\ref{sec:analysis} analyzes when and why AugLift helps, including its interaction with image features and the AugLiftV2 extension that uses learned depth features.
% Finally, Section~\ref{sec:conclusion} discusses limitations and concludes.


==> sec/2_related_work.tex <==
\section{Literature Review}
\label{sec:lit_review}
% ApaarComments#1: Not reviewing; assuming it's unchanged

Research in monocular 3D human pose estimation has progressed along several distinct avenues. In the following, we provide a structured review of the relevant literature along these themes—2D-to-3D lifting, generalization strategies, and weakly supervised learning—before discussing methods that enrich the lifting input, which is most relevant to our work.

\noindent\textbf{2D-to-3D Lifting.}
The paradigm of lifting 2D keypoints to 3D space gained prominence after Martinez et al.~\cite{martinez2017simple} demonstrated that a simple, fully-connected network could achieve competitive results by operating directly on 2D coordinates. This approach, however, struggles with the inherent ambiguity of single-frame inputs. To mitigate this, temporal models were introduced. For instance, VideoPose3D~\cite{pavllo2018video} leverages temporal convolutions over sequences of 2D poses to enforce motion consistency. More recently, Transformer-based architectures like MotionBERT~\cite{zhu2023motionbert} have become state-of-the-art by jointly modeling spatial and temporal relationships in human motion. Despite their success, these foundational methods still face challenges with occlusions and depth ambiguities, motivating the need for richer input signals.

\noindent\textbf{Generalization Strategies.}
Improving generalization to unseen datasets and real-world scenarios remains a primary challenge. Several strategies focus on data augmentation and architectural enhancements. PoseAug~\cite{gong2021poseaug}, for example, uses virtual camera augmentations to simulate multiple perspectives during training, thereby improving robustness. Other works propose multitask learning; Wang et al.~\cite{wang2020predicting} integrate 3D pose estimation with camera viewpoint prediction to leverage complementary information. Rhodin et al.~\cite{rhodin2018unsupervised} use a geometry-aware encoder-decoder framework to learn from multi-view images in a semi-supervised fashion. While effective, these methods often introduce significant architectural complexity or require specialized training data.

\noindent\textbf{Weakly-Supervised and Unsupervised Learning.}
Given the high cost of acquiring 3D annotations, methods that reduce reliance on labeled data are crucial. Unsupervised approaches, such as the one by Chen et al.~\cite{chen2019unsupervised}, enforce geometric self-consistency through a lift-reproject-lift cycle, using a 2D pose discriminator to ensure plausible skeletons without any 3D priors. Semi-supervised techniques, explored by Pavllo et al.~\cite{pavllo2018video}, combine limited 3D ground truth with a larger corpus of 2D data by minimizing a reprojection loss. These methods showcase how geometric constraints can substitute for explicit 3D labels.

% \noindent\textbf{Enriching Lifting with Image-Derived Cues.}
% To overcome the limitations of using only 2D coordinates, another key line of research has explored enriching the input with cues derived directly from the source image. One approach involves creating hybrid models that condition the lifter on rich visual features from a CNN backbone~\cite{nie2019single, xu2022monocular}. However, this strategy faces a critical generalization challenge, as these dense features often learn spurious correlations from the training set's background and appearance~\cite{zhou2023lifting}. To avoid these pitfalls, other works utilize more targeted, semantic signals. For instance, the confidence scores from the 2D detector have been used in isolation to improve robustness to noisy detections~\cite{gong2021poseaug}. Separately, to address depth ambiguity, other methods have incorporated depth-related information, most commonly in the form of relative ordinal rankings~\cite{pavlakos2018ordinal, jiang2021category}. While these works demonstrate that both detection confidence and depth information are valuable signals \textit{in isolation}, their combined potential to boost cross-dataset generalization has remained largely unexplored. Our work, \textit{AugLift}, fills this gap by proposing a simple yet powerful fusion of these two orthogonal cues, demonstrating that their joint use is a critical ingredient for robust, real-world performance.

\noindent\textbf{Enriching Lifting with Image-Derived Cues.}
To overcome the limitations of using only 2D coordinates, another key line of research has explored enriching the input with cues derived directly from the source image. One approach involves creating hybrid models that condition the lifter on rich visual features from a CNN backbone~\cite{nie2019single, xu2022monocular}. However, this strategy faces a critical generalization challenge, as these dense features often learn spurious correlations with the training set's background and appearance~\cite{zhou2023lifting}. To avoid these pitfalls, other works utilize more targeted, semantic signals. For instance, the confidence scores from a 2D detector have been used in isolation to improve robustness to noisy detections~\cite{gong2021poseaug}. Separately, other methods incorporate depth-related information---most commonly as relative ordinal rankings~\cite{pavlakos2018ordinal, jiang2021category}---to address depth ambiguity. We, by contrast, study compact local depth descriptors computed from monocular depth predictions, which improve generalization. As we later show, these sparse descriptors are also highly complementary with dense feature fusion.

% A key limitation of these specialized approaches, however, is that they require the true depth information for model training, creating a data bottleneck. In contrast, AugLift bypasses this data bottleneck by harnessing pretrained models with strong generalization. Further, as we shall see the true potential lies not in using isolated cues, but in the joint use of confidence and depth estimate, which is superior to prior art. Examples of our complementary inputs are shown in Figure \ref{fig:depth_confidence}.% \
% \niko{revise the last sentence or two}
% 

==> sec/3_method_tmp.tex <==
\vspace{-10pt}
\section{Methods} 
\label{sec:methods}

\subsection{Motivation} 
\label{ssec:prelim_analyses}
The design of AugLift was guided by preliminary analyses aimed at understanding the failure modes of modern lifting models.

\noindent\textbf{Motion Cues Can Harm Generalization.}
A common assumption in 3D HPE is that temporal information should improve performance.
Our investigation challenges this assumption in the context of cross-dataset generalization.
To isolate the effect of motion dynamics from detection noise, this analysis was performed using ground-truth 2D keypoints.
While longer motion sequences consistently reduce in-distribution error, we found that they typically \emph{degrade} performance on out-of-distribution datasets (see Appendix, Fig.~\ref{fig:sequence_length_generalization_TCN}).
To probe this further, we tested models on \emph{novel motions composed of familiar poses} (e.g., reversed or sped-up actions) and again observed a significant performance drop.
This indicates that temporal models overfit to the limited motion dynamics present in the training data.
We conjecture this occurs because the combinatorial space of valid human motions is vastly larger than the space of static poses, making it difficult to generalize from the motion examples in current datasets.
These findings underscore the need for richer per-frame features to improve generalization.

\noindent\textbf{Per-Frame Depth Cues Offer a Robust Alternative.}
Motivated by this, we investigated the potential of enriching the per-frame input instead.
In contrast to prior works that rely on generic image-derived cues (see Section~\ref{sec:lit_review}), our analysis focused on \textit{depth cues} as a particularly promising signal.
To estimate their upper bound, we conducted oracle experiments using privileged \emph{ground-truth ordinal depth} information at varying granularities.
The results were compelling: augmenting the sparse $(x,y)$ input with even coarse, three-bin ordinal depth information reduced cross-dataset error (H3.6M$\rightarrow$3DPW) by approximately $25\%$ (see Appendix, Table~\ref{tab:coarse_od_generalization_vp3d}).
This suggests that providing the lifter with even basic geometric context via depth cues is a powerful and robust path toward better generalization.



\begin{algorithm}[t]
\caption{The AugLift module.}
\label{alg:auglift_pipeline}
\small
\textbf{Input:} Image $I$ containing the human subject.

\begin{algorithmic}
    \STATE \textbf{Step 1: Obtain 2D keypoints with confidence scores}
    \STATE \textit{This step is identical to standard lifting.} Run a 2D keypoint detector on $I$ to obtain keypoints with confidence,
    $\{(x_j, y_j, c_j)\}_{j=1}^K$.

    \vspace{5pt}\STATE \textbf{Step 2: Obtain a monocular depth map}
    \STATE Run an off-the-shelf monocular depth estimator on $I$ to obtain a depth map $D$ defined on image pixels.

    \vspace{5pt}\STATE \textbf{Step 3: Compute confidence-aware local depth statistics}
    \FOR{$j = 1, \ldots, K$}
        \STATE \hspace{5pt} i. Convert confidence $c_j \in [0,1]$ to a sampling radius \\
        \hspace{15pt} $r_j = r_{\min} + (1 - c_j)\,(r_{\max} - r_{\min})$.
        \STATE \hspace{5pt} ii. Clamp $r_j$ to $[r_{\min}, r_{\max}]$.
        \STATE \hspace{5pt} iii. Define
        $\mathcal{N}_j = \{(u,v) : \|(u,v) - (x_j,y_j)\|_2 \le r_j\}$.
        \STATE \hspace{5pt} iv. Collect depth values $\mathcal{D}_j = \{D(u,v) \mid (u,v) \in \mathcal{N}_j\}$.
        \STATE \hspace{5pt} v. Compute depth statistics $d_j = \operatorname{median}(\mathcal{D}_j)$, \\
        \hspace{15pt}  $d^{\min}_j = \min(\mathcal{D}_j)$, $d^{\max}_j = \max(\mathcal{D}_j)$.
    \ENDFOR

    \vspace{5pt}\STATE \textbf{Step 4: Rescale 2D keypoints per normalized bounding box}
    \STATE \hspace{5pt} i. Compute keypoint centroid: $c = \bigl(\frac{1}{K}\sum_j x_j, \;\frac{1}{K}\sum_j y_j\bigr)$.
    \STATE \hspace{5pt} ii. Compute box size (average of width and height): \\
        \hspace{15pt} $b = \frac{1}{2}\bigl[(\max_j x_j - \min_j x_j) + (\max_j y_j - \min_j y_j)\bigr]$.
    \STATE \hspace{5pt} iii. Compute scale factor $s =\bar{b}/b$, where $\bar{b}$ is the mean training-set box size.
    \STATE \hspace{5pt} iv. Update $(x_j, y_j) := s \cdot \bigl((x_j, y_j) - c\bigr) + c$ for all $j$.

    \vspace{5pt}\STATE \textbf{Step 5: Normalize confidence and depth statistics}
    \STATE \hspace{5pt} i. Rescale confidence to $[-1,1]$: $\tilde c_j = 2c_j - 1$ for all $j$.
    \STATE \hspace{5pt} ii. Obtain root-relative depths: $\tilde d_j=d_j - d_{\text{root}}$ for all $j$.
    \STATE \hspace{5pt} iii. Clip root-relative depths so $\tilde d_j \in [- \tilde d_{\max}, \tilde d_{\max}]$ for all $j$.
\end{algorithmic}

\textbf{Output:} 6D feature vector
$\tilde q_j = (x_j, y_j, \tilde c_j, \tilde d_j, \tilde d^{\min}_j, \tilde d^{\max}_j)$
for keypoints $j = 1,\ldots,K$. These augmented features serve as inputs to the lifting model.
\end{algorithm}
\vspace{-5pt}
\vspace{-5pt}

\subsection{The AugLift Method}
\label{ssec:auglift_method}

The AugLift method is a lightweight pre-processing pipeline designed to be a modular add-on to any existing lifting-based model.
It transforms the standard 2D keypoint inputs into a richer 6D representation that incorporates both confidence and local depth statistics, without altering the core lifting architecture.
The full procedure is summarized in Algorithm~\ref{alg:auglift_pipeline}.

\noindent\textbf{From 2D keypoints to UADD.}
Given an input image $I$, we first run a standard 2D keypoint detector to obtain keypoints and their confidences $\{(x_j, y_j, c_j)\}_{j=1}^K$.
We then run a single off-the-shelf monocular depth estimator on $I$ to obtain a dense depth map $D$.
For each joint $j$, we define a \emph{confidence-aware} radius
\[
    r_j = r_{\min} + (1 - c_j)\,(r_{\max} - r_{\min}),
\]
clamped to the range $[r_{\min}, r_{\max}]$, and construct a local neighborhood
$\mathcal{N}_j = \{(u,v) : \|(u,v) - (x_j,y_j)\|_2 \le r_j\}$.
We collect the corresponding depth values $\mathcal{D}_j = \{D(u,v) \mid (u,v) \in \mathcal{N}_j\}$ and compute three summary statistics:
a robust central estimate $d_j$ (median of $\mathcal{D}_j$), the minimum $d^{\min}_j$, and the maximum $d^{\max}_j$.
Together with the detector confidence $c_j$, these form the \emph{Uncertainty-Aware Depth Descriptor} (UADD)
\[
    \text{UADD}_j = (c_j, d_j, d^{\min}_j, d^{\max}_j).
\]

Intuitively, $d^{\min}_j$ captures the depth of the nearest occluding surface and acts as a lower bound on the true joint depth, while $d^{\max}_j$ reflects more distant surfaces and background clutter.
The median $d_j$ provides a robust estimate of the typical depth in the neighborhood, which is close to the true joint depth when the joint is visible.
The confidence $c_j$ controls the neighborhood size: for high-confidence joints we use a small radius and rely on precise, localized depth; for low-confidence (often occluded) joints we expand the radius to gather a broader, more conservative depth signal.
This confidence-aware sampling turns a single depth value into a compact descriptor that captures both local geometry and its reliability.

\noindent\textbf{Normalization and integration into lifting.}
Before being passed to the lifting model, we apply two normalization steps.
First, to handle variations in camera distance between training and test scenes, we standardize the skeleton scale by applying a bounding-box rescaling transformation to the $(x_j,y_j)$ coordinates, as in Step~4 of Algorithm~\ref{alg:auglift_pipeline}.
Second, we normalize the new channels: confidence is mapped to $[-1,1]$ via $\tilde c_j = 2c_j - 1$, and depth statistics are made root-relative and clipped to a maximum absolute value of $\tilde d_{\max}$. This helps, for example, to assign a reasonable no-information default when dropout zeroes out the confidence signal at training. In our experiments, we use a neighborhood radius between $r_{\min}=3$ pixels and $r_{\max}=30$ pixels for sampling depth values and a maximum relative depth of $\tilde d_{\max}=2$ meters. The final per-joint input is therefore
\[
    \tilde q_j = (x_j, y_j, \tilde c_j, \tilde d_j, \tilde d^{\min}_j, \tilde d^{\max}_j),
\]
a 6D feature vector that augments the original 2D coordinates with UADD.

Integrating AugLift into an existing lifting model requires only a minimal architectural change: the input layer is widened from $2K$ channels to $6K$, while all subsequent layers, training losses, and optimization remain unchanged.
With this pre-processing in place, the modified lifting model is trained on the original training data and evaluated strictly in the detection setting (using detected rather than ground-truth 2D keypoints), which both minimizes the domain gap to real-world usage and is necessary to obtain meaningful confidence scores $c_j$ for UADD.












% \subsection{The AugLift Method}
% % ApaarComments#1: This needs to be updated. Specifically, there should be a single subsection describing our method (currently this seems split across this and the next subsection). We can refer to the info added by AugLift as a "uncertainty-aware depth descriptor", which consists of the (c, d, d_max, d_min) for each keypoint.

% The AugLift method is a lightweight pre-processing pipeline designed to be a modular add-on to any existing lifting-based model. It transforms the standard 2D keypoint inputs into a richer 4D representation to improve generalization, without altering the core lifting architecture. The full procedure is detailed in Algorithm~\ref{alg:auglift_pipeline}.

% The core of AugLift is the augmentation of each 2D keypoint $(x_j, y_j)$ with two additional signals: a detector confidence score $c_j$ and a metric depth estimate $d_j$. The confidence score, provided directly by the 2D detector, serves as a powerful proxy for joint visibility and reliability. The depth estimate is sourced from an off-the-shelf monocular depth estimation model. To ensure robustness against noise and occlusions, we don't just sample the depth at the keypoint's exact location; instead, as shown in Step 2 of Algorithm~\ref{alg:auglift_pipeline}, we take the minimum depth value in a small local neighborhood. This captures the depth of the nearest occluding surface, providing a more reliable geometric cue. It is crucial to interpret this signal correctly: for an occluded keypoint, this value serves as a robust lower bound on its true depth, while for a visible keypoint, it provides a precise metric estimate—a much richer signal than the relative ordinal rankings used in prior work.

% Before being passed to the lifting model, the inputs undergo two normalization procedures that help improve generalization. First, to handle variations in camera distance from those seen at training, we standardize the skeleton's scale by applying a bounding box rescaling transformation to the $(x,y)$ coordinates (Step 3). Second, the new feature channels are normalized (Step 4): confidence is mapped to $[-1, 1]$, and the depth values are made root-relative and clipped to a maximum value, $d_{\max}$. This helps, for example, assign a reasonable no-information default when dropout zeroes out the confidence signal at training. In our experiments, we use a neighborhood radius of $r=3$ pixels for depth sampling and a maximum relative depth of $d_{\max}=2$ meters.

% Integrating this final 4D input vector requires only a minimal change to the lifting model: the input layer's width is simply expanded to accept $4K$ channels instead of the original $2K$, leaving all deeper layers untouched.

% With the AugLift pre-processing in place, the modified lifting model is then trained using the original training data. All training and inference are performed in the detection setting (i.e., using detected, not ground-truth, 2D keypoints). This is essential for two reasons: it minimizes the domain gap to real-world scenarios, and it is a prerequisite for our method, as the confidence score $c_j$ is only defined for detected keypoints.

% \subsection{Confidence-Aware Depth Uncertainty Sampling}
% We don’t just concatenate off the shelf signals. We design a modular architecture that incorporates uncertainty sampling of depth signals from the monocular depth map based on the 2D keypoint confidence.



% The core AugLift method described in Section~3.2 uses a fixed neighborhood $r$ to sample the depth $d$. While effective, this approach treats all keypoints uniformly, regardless of their reliability. A confident keypoint (e.g., a clear, visible torso) and an unconfident keypoint (e.g., a heavily occluded foot) are both sampled with the same logic.

% To address this, we make the sampling process confidence-aware. Instead of sampling only the minimum depth, we create a richer local descriptor that captures the uncertainty of the depth map in each keypoint's neighborhood. The core idea is to vary the sampling neighborhood inversely with the 2D keypoint confidence score $c$:

% \begin{itemize}
%     % ApaarComments#1: I don't think we need to be so explicit/verbose with explaining our core idea; the previous sentence is already quite clear. We could just say "For example, .." to explain the gist of it.
%     \item \textbf{High Confidence ($c$):} The 2D keypoint is reliable, so we trust the depth map at its location. We sample from a small neighborhood, capturing a precise local depth.
%     \item \textbf{Low Confidence ($c$):} The 2D keypoint is unreliable (likely occluded or noisy). We do not trust the depth at this specific pixel, so we sample from a wider neighborhood and compute summary statistics (e.g., minimum, maximum) across this larger patch.
% \end{itemize}

% This process replaces the single depth value $d$ with a small feature vector representing the local depth distribution. The resulting \textbf{uncertainty-aware descriptor} provides the lifting model with a richer geometric signal, allowing it to distinguish between a \textit{confidently near} keypoint and a \textit{confidently occluded} one (where the depth signal itself is noisy). Despite its expressiveness, this descriptor remains lightweight and generalizable. In contrast to this small, interpretable depth descriptor, we also investigate the use of richer image and depth feature maps fused with the lifting model in Section~\ref{}. \niko{fix reference}
% % ApaarComments#1: Should we fold all the augmenting data into the "uncertainty-aware descriptor"? This would include confidence and all depth-related quantities. Decision: yes, UADD should refer to (c, d, d_min, d_max)



==> sec/4_experiments_tmp.tex <==

\section{Experiments}
\label{sec:experiments}





\vspace{-2pt}
\setlength{\intextsep}{-4pt} % vertical space above & below [h] floats

\subsection{Experimental Setup}\label{ssec:expt_setup}

% \niko{replace with some of our posthoc analysis style figures 2-3, and or move to appendix.}
\begin{figure}[tb]
    \centering

    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/qual-1.png}
    \end{minipage}
    \hspace{8mm}
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/qual-2.png}
    \end{minipage}

    \vspace{3mm}

    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/qual-5.png}
    \end{minipage}
    \hspace{8mm}
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/qual-4.png}
    \end{minipage}

    \caption{\textbf{Qualitative results demonstrating AugLift's robustness to ambiguity}. These visualizations compare the baseline (Vanilla Pred, red) with our AugLift-enabled model (Ours Pred, green) against the ground truth (black). The baseline, relying on sparse 2D keypoints alone, fails on challenging, out-of-distribution poses with significant occlusion (e.g., sitting, crouching). AugLift, through its Uncertainty-Aware Depth Descriptors (UADDs), adaptively weighs geometric cues and keypoint reliability to resolve front–back ambiguities and recover a more accurate 3D structure.}
    \label{fig:qualitative_results}
\end{figure}




\noindent\textbf{Datasets.}
We conduct experiments on four diverse 3D HPE datasets: Human3.6M (H36M)~\cite{ionescu2014human3}, MPI-INF-3DHP (3DHP)~\cite{mehta2016monocular}, Fit3D~\cite{fieraru2021alfit}, and 3D-Pose-in-the-Wild (3DPW)~\cite{vonmarcard2018recovering}. Each dataset offers unique challenges: H36M consists of controlled indoor motions, 3DHP has greater viewpoint diversity, Fit3D contains varied fitness motions, and 3DPW is a challenging in-the-wild dataset with complex activities and dense occlusions. To thoroughly evaluate generalization, we use H36M, 3DHP, and Fit3D for both training and testing, leveraging their corresponding splits. Due to its smaller size, 3DPW is used exclusively as a test set. While we train on different datasets, H36M serves as our default training set for experiments where the training data is fixed.

\noindent\textbf{Lifting Architectures.}
To demonstrate that AugLift is a modular add-on, we integrate it into four representative lifting backbones: the Transformer-based MotionBERT~\cite{zhu2023motionbert} and PoseFormer~\cite{Zheng2021PoseFormer}, the TCN-based VideoPose3D~\cite{pavllo2018video}, and the MLP-based SimpleBaseline~\cite{martinez2017simple}. Together, these popular models represent a diverse range of lifting paradigms, from simple MLPs and temporal convolutions to state-of-the-art Transformers. As a recent, state-of-the-art model, MotionBERT serves as our default lifting architecture for cross-dataset experiments.

\noindent\textbf{Evaluation Protocol.}
Following standard practice, we measure performance using Mean Per Joint Position Error (MPJPE) in millimeters. We report both in-distribution (ID) performance on the validation split of the training dataset and out-of-distribution (OOD) performance on other datasets to assess generalization. Crucially, all main experiments are conducted in the ``detection setting,'' where models are trained and tested on 2D keypoints produced by a detector, not ground truth. This aligns our evaluation with real-world application. To ensure a fair and unified comparison, we use a single off-the-shelf 2D detector (RTMPose-L~\cite{jiang2023rtmpose}) and depth estimation model (Depth Anything v2~\cite{depthanythingv2}) for all experiments. Accordingly, we train both the original backbones and their AugLift-enabled counterparts on the keypoints produced by this detector. As a result, our baseline MPJPE scores may differ slightly from those reported in prior work, which rely on H36M-tuned detectors or ground-truth keypoints that are incompatible with our protocol.

% \vspace{8pt}
\begin{table}[!t]
\renewcommand{\arraystretch}{0.95}
\centering
\caption{
\textbf{AugLift improves both cross-dataset (OOD) and in-distribution (ID) performance, regardless of the training dataset.} We show raw MPJPE (mm) for the MotionBERT baseline versus the AugLift-enabled model when trained on three different source datasets. The mean improvement is 10.1\% for OOD and 4.0\% for ID settings.
}
\begin{tabular}{l l r r r r}
\toprule
Train DS & Variant       & H36M   & 3DHP  & Fit3D & 3DPW  \\
\midrule
H36M     & Baseline      & 41.8   & 96.7  & 66.6  & 154.8 \\
         & AugLift       & 40.7   & 85.9  & 55.8  & 146.9 \\
         & $\Delta_{\text{ID}}$  & \textbf{2.6\%} & --          & --          & --          \\
         & $\Delta_{\text{OOD}}$ & --              & \textbf{11.2\%} & \textbf{16.2\%} & \textbf{5.1\%} \\
\midrule
3DHP     & Baseline      & 80.9   & 52.2  & 88.2  & 130.3 \\
         & AugLift       & 79.3   & 50.9  & 76.8  & 121.3 \\
         & $\Delta_{\text{ID}}$  & --              & \textbf{2.5\%}  & --              & --              \\
         & $\Delta_{\text{OOD}}$ & \textbf{2.0\%}  & --              & \textbf{12.9\%} & \textbf{6.9\%}  \\
\midrule
Fit3D    & Baseline      & 127.4  & 166.1 & 39.9  & 195.4 \\
         & AugLift       & 109.1  & 132.9 & 37.1  & 191.3 \\
         & $\Delta_{\text{ID}}$  & --              & --              & \textbf{7.0\%}  & --              \\
         & $\Delta_{\text{OOD}}$ & \textbf{14.4\%} & \textbf{20.0\%} & --              & \textbf{2.1\%}  \\
\bottomrule
\end{tabular}
\label{tab:motionbert_quad}
\end{table}


\subsection{Cross-Dataset Study}

\emph{Does AugLift improve performance on unseen datasets? Does it help—or harm—accuracy on the source dataset itself?} We conduct a rigorous study to answer these questions.

\noindent\textbf{Setup.} We train a baseline lifting model and its AugLift-enabled counterpart in three independent training runs, each on a different source dataset—H36M, 3DHP, and Fit3D. After training, every model is evaluated on all four datasets (H36M, 3DHP, Fit3D, 3DPW), in line with our Evaluation Protocol in Section~\ref{ssec:expt_setup}. This yields one ID and three OOD scores per run. Using three distinct training distributions ensures our findings are robust and not biased by a single dataset. For this study, we use the state-of-the-art MotionBERT backbone.

\noindent\textbf{Results.} Table~\ref{tab:motionbert_quad} shows that \textbf{AugLift improves accuracy in every ID and OOD scenario}. Averaged across all three training regimes, AugLift improves OOD performance by a mean of \textbf{10.1\%} and also boosts ID performance by a mean of \textbf{4.0\%}. The OOD gains are most pronounced under large domain shifts; for example, training on Fit3D and testing on 3DHP yields a 20.0\% error reduction. These findings demonstrate that AugLift is a powerful mechanism for improving generalization without sacrificing in-domain accuracy.



\subsection{Cross-Architecture Study}\label{ssec:cross_arch_study}

\begin{table}[tb]
\vspace{-2pt}        
\centering
\caption{\textbf{AugLift provides robust gains across diverse architectures.} Raw MPJPE (mm) on H36M (ID) and three OOD sets. For each backbone, we compare the base lifting model to its AugLift-enabled counterpart. Across all architectures, AugLift yields consistent improvements in both ID and OOD performance. The mean improvement over the baseline is 2.3\% for ID and 8.9\% for OOD performance.}
% \caption{\textbf{AugLift provides robust gains across diverse architectures, and the synergy of confidence and depth is critical.} Raw MPJPE (mm) on H36M (ID) and three OOD sets. Adding only confidence provides marginal benefits, while the full AugLift model delivers significant ID and OOD improvements across all backbones. The mean improvement for AugLift over the baseline is 2.3\% for ID and 8.9\% for OOD performance.}
\begin{tabular}{l l rr | rrrr}
\hline
Architecture         & Variant                   & \multicolumn{2}{c|}{In‑Distribution}      & \multicolumn{4}{c}{Out‑of‑Distribution}                \\
\cline{3-8}
                     &                           & H36M         & $\Delta_{\mathrm{ID}}$ (\%) & 3DHP         & Fit3D        & 3DPW         & $\Delta_{\mathrm{OOD}}$ (\%) \\
\hline
MotionBERT           & Base Model                & 41.8         & ---                         & 96.7         & 66.6         & 154.8        & ---                          \\
                     % & Base Model + confidence         & 41.3         & ---                         & 92.6         & 63.6         & 151.0        & ---                          \\
                     & Base Model + AugLift      & \textbf{40.7} & \textbf{2.6\%}             & \textbf{85.9} & \textbf{55.8} & \textbf{146.9} & \textbf{10.8\%}              \\
\hline
SimpleBaseline       & Base Model                & 57.5         & ---                         & 103.8        & 81.6         & 183.7        & ---                          \\
                     % & Base Model + confidence         & 58.5         & ---                         & 101.4        & 84.0         & 167.5        & ---                          \\
                     & Base Model + AugLift      & \textbf{54.6} & \textbf{5.0\%}             & \textbf{96.1} & \textbf{75.2} & \textbf{147.4} & \textbf{11.7\%}              \\
\hline
VideoPose3D          & Base Model                & 53.9         & ---                         & 93.6         & 79.2         & 153.4        & ---                          \\
                     % & Base Model + confidence         & 55.0         & ---                         & 93.5         & 80.5         & 146.2        & ---                          \\
                     & Base Model + AugLift      & \textbf{53.8} & \textbf{0.2\%}             & \textbf{89.8} & \textbf{75.5} & \textbf{140.8} & \textbf{5.7\%}               \\
\hline
PoseFormer           & Base Model                & 50.5         & ---                         & 90.6         & 75.3         & 135.6        & ---                          \\
                     % & Base Model + confidence         & 51.3         & ---                         & 90.6         & 76.0         & 129.7        & ---                          \\
                     & Base Model + AugLift      & \textbf{49.8} & \textbf{1.4\%}             & \textbf{83.8} & \textbf{70.2} & \textbf{124.5} & \textbf{7.6\%}               \\
\hline
\end{tabular}
\label{tab:full_results_aug}
\end{table}
\vspace{-2pt}        

\emph{Do the gains from AugLift span different lifting architectures?} Having established that AugLift provides robust generalization across datasets, we establish the same across model architectures.

\noindent\textbf{Setup.} We evaluate four distinct and popular lifting backbones: SimpleBaseline, VideoPose3D, PoseFormer, and MotionBERT, as detailed in Section~\ref{ssec:expt_setup}. For each backbone, we train the standard baseline and the full AugLift-enabled model. All models in this study are trained on H36M and evaluated on both in-distribution (H36M) and out-of-distribution (3DHP, Fit3D, and 3DPW) test sets.

\noindent\textbf{Results.} Table~\ref{tab:full_results_aug} confirms that \textbf{AugLift consistently improves performance across all four architectures}. On average, AugLift reduces OOD error by \textbf{8.9\%} and ID error by \textbf{2.3\%}. Notably, the simplest model, SimpleBaseline, receives one of the largest OOD improvements at 11.7\%, suggesting that the explicit geometric cues provided by AugLift may be particularly beneficial for models with less capacity to learn such relationships implicitly.

% Furthermore, this \textbf{experiment highlights the critical synergy between the confidence and depth cues}. As shown in Table~\ref{tab:full_results_aug}, augmenting the baseline models with only confidence scores yields negligible or inconsistent gains. The significant and consistent performance boost is only unlocked when both confidence and depth are used jointly: the depth offers a precise signal for visible keypoints and a lower-bound for occluded ones, while the confidence (which strongly correlates with keypoint visibility) helps distinguish between these two cases. It is this fusion of a reliability signal (confidence) with a geometric signal (depth) that provides the rich, robust input needed for generalized 3D pose estimation.



% \begin{minipage}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{qual-7.png}
% \end{minipage}
% \hfill
% \begin{minipage}{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{qual-3.png}
% \end{minipage}
% \vspace{-4pt}        
% \caption{\textbf{Qualitative comparison of a baseline model versus the AugLift-enabled model on challenging poses.} In these examples, MotionBert was trained on H36M and tested on the OOD 3DHP dataset. The ground truth pose is shown in black, the baseline prediction in red, and the AugLift prediction in green. AugLift consistently produces more accurate 3D poses, especially for ambiguous scenarios like sitting and crouching where its additional depth and confidence cues are most vital.}
% \label{fig:xycd_examples}
% % \vspace{-8pt}        
% \end{figure}



\subsection{Ablations}
\label{sec:ablations_summary}
\noindent\textbf{Setup.} We conduct ablations along three axes: (i) removing depth and using confidence only, (ii) disabling our per-instance bounding box rescaling, and (iii) varying the temporal context by sweeping the sequence length from 1 to 243 frames. Full results and discussion are provided in Appendix F.

\noindent\textbf{Results.} In summary, using confidence alone yields negligible or inconsistent gains, whereas adding depth on top of confidence produces the strong, consistent ID/OOD improvements reported in Tables~\ref{tab:motionbert_quad} and \ref{tab:full_results_aug}, underscoring the importance of geometric depth cues. Bounding box rescaling delivers substantial improvements on 3DPW (e.g., up to 14.3\% error reduction in Appendix Table~\ref{tab:bbox-rescaling}) and is broadly beneficial even without UADD, making it a generally useful component for handling train–test scale shifts. Finally, the sequence-length study (Appendix Table~\ref{tab:improvements_fixed}) shows that while ID gains taper with longer temporal context, AugLift’s OOD gains remain large across all sequence lengths, confirming that its per-frame depth cues are complementary to motion and effective in both short- and long-horizon regimes.


\begin{table}[t]
    \centering
    \caption{\textbf{AugLift's gains are largest on novel, out-of-distribution poses.} To understand why AugLift improves out-of-distribution (OOD) performance, we analyze its gains on Fit3D (trained on H36M) by stratifying test frames based on their 3D pose similarity to the H36M training set. The baseline model (XY), which can only rely on brittle pose priors learned from H36M, fails on novel poses, with error increasing to 109.2 MPJPE on the "Lowest 20\%" similarity bucket. AugLift, however, reduces the error by a significant 15.7\%. MPJPE reported for each model.}
    \label{tab:domain_similarity_fit3d}
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Similarity Bucket} & \textbf{Base} & \textbf{AugLift} & \textbf{$\Delta$ (\%)} \\
        \midrule
        Highest 20\%  & 55.8  & 53.6  & -3.9\% \\
        Middle 60\%   & 67.3  & 66.1  & -1.9\% \\
        Lowest 20\%   & 109.2 & 92.1  & -15.7\% \\
        \bottomrule
    \end{tabular}
    % \vspace{}
\end{table}
\vspace{-5pt}


\subsection{When and Why Does AugLift Help?}
\label{ssec:when_why}

\noindent\textbf{Setup.}
To understand where AugLift’s gains come from, we perform a post-hoc analysis using a PoseFormer model (sequence length 27) trained on H36M and evaluated with and without AugLift on three OOD test sets: Fit3D, 3DHP, and 3DPW.
We design three analyses, each targeting a specific challenge in 3D pose estimation.
In each case, we bucket test frames using an oracle metric and compare the baseline and AugLift within each bucket:
\begin{itemize}
    \item \emph{Occlusion status.} To measure the impact of self-occlusion, we stratify test frames into quartiles (Q1–clear to Q4–most occluded) using a geometric occlusion proxy derived from the ground-truth 3D pose, which detects 2D keypoint overlap based on 3D depth ordering.
    \item \emph{Pose similarity.} To quantify how AugLift behaves on poses not seen in training, we cluster H36M training poses into a set of 3D prototypes and, for each test frame, compute the distance to the nearest prototype. This defines three buckets: “Highest 20\%”, “Middle 60\%”, and “Lowest 20\%” similarity (Table~\ref{tab:domain_similarity_fit3d}).
    \item \emph{2D keypoint reliability.} To probe robustness to noisy inputs, we measure mean 2D error (pixels) between detected and ground-truth keypoints and stratify frames into quartiles from “Q1–Best” (lowest 2D error) to “Q4–Worst” (highest 2D error).
\end{itemize}
We complement these quantitative analyses with qualitative examples in Figure~\ref{fig:qualitative_results} on challenging poses such as sitting and crouching.
% \vspace{-5pt}

\noindent\textbf{Findings.}
We observe three consistent patterns:
% \vspace{-2pt}
\begin{itemize}
    \item \emph{Tail-error reduction.} AugLift primarily reduces worst-case failures: on 3DHP, p90 error drops by 11.1\% (154.1\,mm $\rightarrow$ 136.9\,mm), while the median (p50) improves by only 3.5\% (80.6\,mm $\rightarrow$ 77.8\,mm), with a similar pattern on 3DPW.
    \item \emph{Occlusion sensitivity.} Gains grow with occlusion. On Fit3D, the least occluded quartile sees a 4.1\% median improvement (64.5\,mm $\rightarrow$ 61.9\,mm), versus 9.4\% (79.6\,mm $\rightarrow$ 72.1\,mm) in the most occluded quartile.
    \item \emph{Pose novelty.} AugLift helps most on poses farthest from the H36M training distribution. On Fit3D (Table~\ref{tab:domain_similarity_fit3d}), the “Lowest 20\%” similarity bucket achieves a 15.7\% MPJPE reduction (109.2\,mm $\rightarrow$ 92.1\,mm), compared to 3.9\% and 1.9\% in the highest and middle buckets.
\end{itemize}
% \vspace{-5pt}
% \vspace{-5pt}

\noindent\textbf{Mechanism: confidence–depth synergy.}
These trends, together with the qualitative examples in Figure~\ref{fig:qualitative_results}, support a simple mechanism view.
When 2D confidence is very low and keypoints are badly misplaced, both the baseline and AugLift can fail, since depth is sampled around the wrong location.
For \emph{moderate} confidence, typically corresponding to partially occluded joints, AugLift provides its largest gains: the $d_{\min}$ statistic acts as a lower bound on true joint depth, helping avoid front--back flips even when the keypoint location is uncertain.
Finally, AugLift can help even for \emph{high}-confidence joints, where 2D locations are accurate but depth remains ambiguous (e.g., bending forward vs.\ backward). Here, the median depth $d$ closely tracks the true joint depth and resolves this ambiguity.
In all regimes, confidence controls the neighborhood size and determines whether depth should be treated as a precise estimate or a conservative bound, making AugLift especially beneficial on occluded, novel, and depth-ambiguous poses.





% \subsection{When and Why Does AugLift Help?}
% \label{ssec:when_why}

% To understand where AugLift’s gains come from, we analyze a PoseFormer model with sequence length 27 trained on H36M, evaluated with and without AugLift on the three OOD test sets (Fit3D, 3DHP, 3DPW). We stratify test frames by (i) self-occlusion level, (ii) pose similarity to the H36M training set, and (iii) 2D keypoint reliability, and we complement this with qualitative examples in Figure~\ref{fig:qualitative_results} and the pose-similarity breakdown in Table~\ref{tab:domain_similarity_fit3d}. Our main findings are:
% \begin{itemize}
%     \item \textbf{Tail-error reduction.} AugLift primarily reduces worst-case failures: on 3DHP, p90 error drops by 11.1\% (154.1\,mm $\rightarrow$ 136.9\,mm), while the median (p50) improves by only 3.5\% (80.6\,mm $\rightarrow$ 77.8\,mm), with a similar pattern on 3DPW.
%     \item \textbf{Occlusion sensitivity.} Gains grow with occlusion. On Fit3D, the least occluded quartile sees a 4.1\% median improvement (64.5\,mm $\rightarrow$ 61.9\,mm), versus 9.4\% (79.6\,mm $\rightarrow$ 72.1\,mm) in the most occluded quartile.
%     \item \textbf{Pose novelty.} AugLift helps most on poses that are farthest from the H36M training distribution. On Fit3D (Table~\ref{tab:domain_similarity_fit3d}), the “Lowest 20\%” similarity bucket achieves a 15.7\% MPJPE reduction (109.2\,mm $\rightarrow$ 92.1\,mm), compared to 3.9\% and 1.9\% in the highest and middle buckets.
% \end{itemize}

% These trends, together with the qualitative examples in Figure~\ref{fig:qualitative_results}, support a simple mechanism view. When 2D confidence is very low and keypoints are badly misplaced, both the baseline and AugLift can fail, since depth is sampled around the wrong location. For \emph{moderate} confidence, typically corresponding to partially occluded joints, AugLift provides its largest gains: the $d^{\min}$ statistic acts as a lower bound on true joint depth, helping avoid front--back flips even when the keypoint location is uncertain. For \emph{high}-confidence joints, where 2D locations are accurate but depth remains ambiguous (e.g., bending forward vs.\ backward), the median depth $d$ closely tracks the true joint depth and resolves this ambiguity. In all cases, confidence controls the neighborhood size and determines whether depth should be treated as a precise estimate or a conservative bound, making AugLift especially beneficial on occluded, novel, and depth-ambiguous poses.





% \subsection{When and Why Does AugLift Help?}
% \label{ssec:when_why}

% To better understand AugLift's behavior, we perform a post-hoc analysis using a PoseFormer model with sequence length 27 trained on H36M, and evaluate it with and without AugLift on the three OOD test sets (Fit3D, 3DHP, 3DPW). We design three oracle-based analyses that bucket test frames by (i) self-occlusion level, (ii) pose novelty relative to the H36M training set, and (iii) 2D keypoint reliability. Full details and plots are provided in Appendix~C; here we summarize the key findings.

% \noindent\textbf{Gains concentrate on hard, occluded, and novel poses.}
% Across datasets, a large fraction of AugLift’s overall MPJPE reduction comes from the tail of the error distribution: on 3DHP, for example, the p90 error drops by 11.1\% while the median drops by only 3.5\%. Stratifying by a geometric self-occlusion proxy, we observe that gains are modest on clear frames but grow substantially with occlusion; on Fit3D, the median improvement increases from 4.1\% in the least occluded quartile to 9.4\% in the most occluded quartile. Similarly, stratifying frames by their 3D pose similarity to H36M reveals that AugLift helps most on novel poses: on Fit3D, the ``Lowest 20\%'' similarity bucket sees a 15.7\% MPJPE reduction, compared to 3.9\% and 1.9\% for the highest and middle buckets, respectively (Table~\ref{tab:domain_similarity_fit3d}). Finally, grouping by 2D keypoint error shows that gains are largest when detections are moderately noisy (rather than near-perfect or completely unreliable), aligning with our design that targets ambiguous but still informative detections.

% \noindent\textbf{Mechanism: confidence–depth synergy across regimes.}
% These trends are consistent with our qualitative observations in Figure~\ref{fig:qualitative_results} and support a simple mechanism view. When \emph{confidence is very low} and 2D keypoints are badly misplaced, both the baseline and AugLift tend to fail, since the depth neighborhood is centered on the wrong location. For \emph{moderate confidence}, typically corresponding to partially occluded joints, AugLift provides the largest gains: the descriptor’s $d^{\min}$ term acts as a lower bound on true joint depth, helping avoid catastrophic front–back mistakes even when the keypoint location is uncertain. For \emph{high-confidence} joints, where 2D locations are accurate but there remains a depth ambiguity (e.g., bending forward vs.\ backward), the median depth $d$ closely tracks the true depth and resolves these ambiguities. In all cases, confidence controls the neighborhood size, telling the model when depth should be trusted as a precise estimate versus a conservative bound. Taken together, these analyses suggest that AugLift is most beneficial exactly where lifting from sparse 2D is inherently under-constrained: occluded, novel, and depth-ambiguous poses.






% \subsection{Post-Hoc Analysis}

% To better understand the mechanism driving AugLift's generalization gains, we perform a post-hoc analysis to investigate what leads to the reduction in error. This investigation dives deeper into the qualitative results from our cross-dataset study.

% \subsubsection{Setup}

% For this analysis, we use our PoseFormer model with a sequence length of 27, trained on the H36M dataset. We then evaluate its performance (both with and without AugLift) on the three out-of-distribution test sets: Fit3D, 3DHP, and 3DPW.
% We introduce three new analyses, each designed to isolate a specific challenge in 3D pose estimation. In each analysis, we divide the test data into buckets based on an oracle metric and compare the performance of the baseline model versus AugLift within each bucket.

% \begin{itemize}
%     \item \textbf{Occlusion Status:} To measure the impact of self-occlusion, we stratify test frames into quartiles (Q1–Clear to Q4–Most Occluded). This stratification is based on a geometric occlusion proxy derived from the ground-truth 3D pose, which identifies 2D keypoint overlap based on 3D depth ordering.

%     \item \textbf{Frame Similarity:} To quantify how AugLift performs on poses not seen in the training data, we measure dissimilarity from the training set. First, we cluster the entire H36M training set's 3D poses into 100 representative pose clusters. Then, for each test frame, we compute its 3D pose distance to the nearest H36M cluster center. This distance serves as our dissimilarity metric, allowing us to bucket the test data into quintiles: ``Most Similar 20\%'', ``Middle 60\%'', and ``Least Similar 20\%''.

%     \item \textbf{2D Keypoint Reliability:} To test robustness to noisy inputs, we measure the 2D keypoint reliability by computing the Euclidean distance (in pixels) between the detected 2D keypoints (our model's input) and the ground-truth 2D keypoints. We then stratify the test set into quartiles based on this mean 2D error, from ``Q1–Best'' (lowest 2D error) to ``Q4–Worst'' (highest 2D error).
% \end{itemize}

% \subsubsection{Findings}
% Our post-hoc analysis yields four key insights into AugLift's mechanism.

% \paragraph{AugLift Primarily Reduces Tail Error}
% A significant portion of the overall MPJPE gain comes from mitigating the worst-case failures. On 3DHP, the p90 error (the worst 10\% of predictions) is reduced by 11.1\% (from 154.1\,mm to 136.9\,mm), while the median error (p50) is reduced by only 3.5\% (80.6\,mm to 77.8\,mm). This pattern holds on 3DPW, where the p90 error drops by 6.2\% while the median drops by just 3.3\%. This demonstrates that AugLift's primary benefit is not in refining already-good predictions, but in providing a robust geometric prior that prevents catastrophic failures.
% \paragraph{Gains Are Largest on Occluded Frames}
% AugLift's benefits are strongly correlated with occlusion. On Fit3D, we stratified frames into four quartiles based on our geometric occlusion proxy. For the clearest quartile (Q1), AugLift provides a modest 4.1\% median improvement (64.5\,mm to 61.9\,mm). However, for the most occluded quartile (Q4), the median benefit more than doubles to 9.4\% (79.6\,mm to 72.1\,mm). This finding supports our hypothesis that the synergistic (c, d) cues are most valuable when 2D keypoints are ambiguous due to self-occlusion.
% \paragraph{AugLift Generalizes to Dissimilar Poses}
% The method shows the largest gains on poses that are most dissimilar to the H36M training data. On Fit3D, frames in the ``Least Similar 20\%'' quintile saw a 15.7\% MPJPE reduction (109.2\,mm to 92.1\,mm). In contrast, the ``Most Similar 20\%'' and ``Middle 60\%'' buckets saw gains of only 3.9\% and 1.9\%, respectively. This trend is consistent on 3DHP, which saw an 11.3\% improvement on its least similar quintile. This strongly suggests AugLift provides robust geometric priors that help the model generalize beyond the training domain's specific pose distribution.

% \begin{table}[t]
%     \centering
%     \caption{\textbf{AugLift's gains are largest on novel, out-of-distribution poses.} To understand why AugLift improves out-of-distribution (OOD) performance, we analyze its gains on Fit3D (trained on H36M) by stratifying test frames based on their 3D pose similarity to the H36M training set . The baseline model (XY), which can only rely on brittle pose priors learned from H36M, fails on novel poses, with error increasing to 109.2 MPJPE on the "Lowest 20\%" similarity bucket. AugLift, however, reduces the error by a significant 15.7\%. MPJPE reported for each model.}
%     \label{tab:domain_similarity_fit3d}
%     \setlength{\tabcolsep}{3.5pt}
%     \renewcommand{\arraystretch}{0.95}
%     \begin{tabular}{lccc}
%         \toprule
%         \textbf{Similarity Bucket} & \textbf{Base} & \textbf{AugLift} & \textbf{$\Delta$ (\%)} \\
%         \midrule
%         Highest 20\%  & 55.8  & 53.6  & -3.9\% \\
%         Middle 60\%   & 67.3  & 66.1  & -1.9\% \\
%         Lowest 20\%   & 109.2 & 92.1  & -15.7\% \\
%         \bottomrule
%     \end{tabular}
    
% \end{table}

% % \subsubsection{Benefits Are Concentrated in the Appendages}
% % An analysis by body part on Fit3D reveals the benefit is not uniform across the skeleton. The most significant gains are concentrated in the limbs, which are most prone to depth ambiguity. The lower appendages (hips, knees, feet) improved by 11.6\% (a 7.82\,mm reduction), and the upper appendages (shoulders, elbows, wrists) improved by 5.3\% (a 4.


==> sec/5_analysis_tmp.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/cvpr_fig6_v2.png}
%     % \hfill
%     % \includegraphics[width=0.48\linewidth]{figures/feature_map_fusion2.png}
%     \caption{Visualization of feature map fusion. We show the 2D detection bounding box from RTMPose (center) aligned with its corresponding feature map, alongside the feature map from the monocular depth estimation model (right). The L2 norm of channel activations is visualized per coarse patch, with patches sampled at 2D keypoint locations and averaged over the four nearest neighbors. This design maintains the lightweight efficiency of standard lifting models and AugLift, while enabling them to leverage richer spatial cues from image and depth features. 
%     % \niko{clarify this; label source vs generalization img`}
%     }
%     \label{fig:feature_fusion}
% \end{figure}

% \section{Deeper Analysis}
% \label{sec:analysis}

% \subsection{Feature Map Experiments}

% In our main proposal, AugLift uses sparse (c, d) cues. A natural question is how this compares to using richer, dense feature maps sampled from the 2D pose detector or the monocular depth model. In this section, we investigate this comparison and explore if AugLift's sparse cues can be combined with dense features for further gains.

% Most prior works that study generalization in lifting operate strictly in the 2D ground-truth setting (e.g., PoseAug \cite{gong2021poseaug}, Lifting-by-Image \cite{zhou2023lifting}), making them incompatible with real-world noisy detections. CAPoseFormer \cite{zhao2023caposeformer} is one of the few methods using 2D detections, but it focuses on richer in-distribution feature fusion rather than cross-dataset generalization, whereas our goal is to evaluate generalization in the realistic detection setting using noisy 2D keypoints. In line with prior literature, we focus on sequence length of 1 for these experiments.

% \subsubsection{Setup}

% We compare AugLift against baselines and combinations using feature maps from our 2D detector (RTMPose) and depth estimator (DAV2). The setting is fixed to 2D detections (from RTMPose) to study real-world generalization.

% \textbf{Implementation Details:} We sample feature maps from the final feature extractor of each model.
% \begin{itemize}
%     \item \textbf{RTMPose:} The feature map has dimensions $(12, 9, 1024)$.
%     \item \textbf{DAV2:} The feature map has spatial dimensions $(37, 37)$. We downsample its channel dimension using a 1D convolution to 256D for efficiency.
% \end{itemize}

% \textbf{Sampling Strategy:} From these coarse feature maps, we interpolate the patch nearest to each 2D keypoint coordinate. We then sample and average the features from the nearest four spatial embeddings for each keypoint.

% \textbf{Model Integration:} The sampled features are integrated into our PoseFormer lifting model. The features are first passed through a learned linear projection layer and then concatenated with the keypoint embeddings before the spatial transformer encoder.




% \subsubsection{Fusing with Features from Detected Keypoints}


% In this experiment, we use the 2D detected keypoint locations to determine where to sample the feature patches. This represents a realistic scenario where the sampling location is as noisy as the 2D pose itself.

% \textbf{Findings:} We observe two interesting patterns. First, for single-frame models (slen1), combining \textbf{AugLift (XYCD)} with image features (+RTM) yields the best OOD performance (85.6\,mm), suggesting that the image features provide complementary information not present in AugLift's sparse cues. In contrast, combining AugLift with depth features (XYCD+DAV) provides no significant benefit over AugLift alone (88.0\,mm vs 89.0\,mm OOD), indicating that our lightweight sparse depth cue ($d$) already captures most of the useful geometric information from the dense depth map. 

% Second, for sequence models (slen9), the gains from feature maps are muted or even negative. For example, XYCD+RTM (90.6\,mm OOD) performs worse than XYCD alone (87.6\,mm OOD). This suggests that feeding dense image or depth features from many frames can lead to dataset-specific overfitting, reinforcing our hypothesis that lightweight spatial cues like AugLift's provide a more robust signal for generalization in temporal models.

% Fusing AugLift with depth feature maps provides the best in-distribution improvements, while fusing AugLift with image feature maps provides the best out of distribution improvement.

% \begin{table}[t]
%     \centering
%     \small % Makes the font size for the caption and table smaller
%     \caption{\textbf{AugLift's sparse cues are complementary to image and dense depth features.} 
% We analyze fusing our sparse AugLift (UADD) with dense image features (+RTMPose) and explore rich feature fusion in the depth map space, an underexplored area, with our AugLiftV2.}
%     \label{tab:feature_map_fusion_combined}
%     \setlength{\tabcolsep}{3.5pt} % Adjust column spacing
%     \renewcommand{\arraystretch}{0.95} % Adjust row height
%     \begin{tabular}{lcccc}
%     \toprule
%     Config & Val & $\Delta_{\mathrm{ID}}$ (\%) & 3DHP & $\Delta_{\mathrm{OOD}}$ \\
%     \midrule
%     Base Model & 54.3 & -- & 94.5 & -- \\
%     Base Model + RTMPose & 51.1 & +5.9 & 88.1 & +6.8 \\
%     \midrule
%     AugLift & 51.7 & +4.8 & 87.9 & +7.0 \\
%     AugLift + RTMPose & 50.3 & +7.4 & 84.6 & +10.5 \\
%     \midrule
%     AugLiftV2 & 47.9 & +11.8 & 87.1 & +7.8 \\
%     AugLiftV2 + RTMPose & 47.9 & +11.8 & 85.9 & +9.1 \\
%     \bottomrule
%     \end{tabular}

% \end{table}
\vspace{-10pt}






\section{Leveraging Image and Depth Feature Maps}
\label{sec:feature_fusion_section}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/cvpr_fig6_v2.png}
    \caption{\textbf{Sampling dense feature maps at 2D keypoints.}
    We show the 2D detection bounding box from RTMPose (center) aligned with its feature map, alongside the monocular depth feature map (right). We visualize the $\ell_2$ norm of channel activations per coarse patch and sample features at 2D keypoints by averaging the four nearest spatial embeddings. This design preserves the lightweight nature of standard lifting and AugLift while enabling the use of richer spatial cues from image and depth features.}
    \label{fig:feature_fusion}
\end{figure}
% \vspace{-15pt}

\begin{table}[t]
    \centering
    \small
    \caption{\textbf{AugLift’s sparse cues are complementary to dense image and depth features.}
    Results are for PoseFormer (sequence length 1) trained on H36M and evaluated on H36M validation (Val, ID) and 3DHP (OOD).
    RTMPose denotes image features from the 2D detector; AugLiftV2 uses depth-image features.
    }
    \label{tab:feature_map_fusion_combined}
    \setlength{\tabcolsep}{3.5pt}
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{lcccc}
    \toprule
    Config              & Val & $\Delta_{\mathrm{ID}}$ (\%) & 3DHP & $\Delta_{\mathrm{OOD}}$ (\%) \\
    \midrule
    Base Model          & 54.3 & --    & 94.5 & --    \\
    Base Model + RTMPose& 51.1 & +5.9 & 88.1 & +6.8 \\
    \midrule
    AugLift             & 51.7 & +4.8 & 87.9 & +7.0 \\
    AugLift + RTMPose   & 50.3 & +7.4 & 84.6 & +10.5 \\
    \midrule
    AugLiftV2           & 47.9 & +11.8 & 87.1 & +7.8 \\
    AugLiftV2 + RTMPose & 47.9 & +11.8 & 85.9 & +9.1 \\
    \bottomrule
    \end{tabular}
    \vspace{-5pt}
\end{table}
% \vspace{-15pt}


\subsection{Complementarity with Image Features}
\label{ssec:image_features}

AugLift uses sparse, interpretable cues (UADD) attached to 2D keypoints.
In parallel, prior work has shown that fusing dense image features from the 2D detector into the lifter can improve accuracy, especially in the single-frame setting (Lifting-by-Image~\cite{zhou2023lifting}, CAPoseFormer~\cite{zhao2023caposeformer}).
Here we ask: \emph{are these two approaches complementary?}

\noindent\textbf{Setup.} We follow the detection setting from Section~\ref{ssec:expt_setup} and train on H36M. 
We mimic a single-frame CAPoseFormer to utilize image features from RTMPose, both with and without AugLift.
From RTMPose, we extract a coarse feature map and sample features at each detected keypoint location by averaging the four nearest spatial patches (Figure~\ref{fig:feature_fusion}).
% We mimic a single-frame CAPoseFormer to utilize image features from RTMPose, both with and without AugLift
% From RTMPose, we extract a coarse feature map and sample features at each detected keypoint location by averaging the four nearest spatial patches (Figure~\ref{fig:feature_fusion}).
The sampled features are linearly projected and concatenated with the keypoint tokens before the transformer encoder. Other details, including feature map sizes, are provided in Appendix G.

\noindent\textbf{Results.}  Table~\ref{tab:feature_map_fusion_combined} shows three main trends.
First, adding image features alone improves both ID and OOD performance over the base model (e.g., $+5.9\%$ ID and $+6.8\%$ OOD).
Second, AugLift by itself provides comparable gains ($+4.8\%$ ID, $+7.0\%$ OOD).
Third—and most importantly—the combination \textbf{AugLift + RTMPose} is best overall, improving ID by $7.4\%$ and OOD by $10.5\%$.
This establishes that AugLift’s sparse, confidence-aware depth cues and dense image features carry \emph{complementary} information, and that using both yields the strongest cross-dataset performance.

\subsection{AugLiftV2: Learning Depth-Image Features}
\label{ssec:depth_features}

Motivated by the success of image-feature fusion, we next explore whether similar dense features extracted from the \emph{monocular depth image} can further strengthen AugLift.
We define \emph{AugLiftV2} as an extension of AugLift that additionally uses these depth-image features.

\noindent\textbf{Setup.} In AugLiftV2, we sample depth-backbone feature maps at 2D keypoints using the same strategy as before (see Figure~\ref{fig:feature_fusion}) and pass them through a small encoder before concatenation with the keypoint tokens.
Unlike UADD, these depth-image features are learned and no longer directly interpretable as simple statistics $(c, d, d_{\min}, d_{\max})$. Architectural details are deferred to Appendix G.

\noindent\textbf{Results.} As shown in  Table~\ref{tab:feature_map_fusion_combined}, AugLiftV2 yields a stronger ID improvement than AugLift (Val 51.7\,mm $\rightarrow$ 47.9\,mm; $+11.8\%$ vs.\ $+4.8\%$) and slightly better OOD performance (87.9\,mm $\rightarrow$ 87.1\,mm; $+7.8\%$ vs.\ $+7.0\%$).
Moreover, AugLiftV2 remains complementary to image features: combining AugLiftV2 with RTMPose improves OOD error from 88.1\,mm to 85.9\,mm ($+9.1\%$ over the base model), while preserving the strong ID gains.
Overall, AugLiftV2 demonstrates that richer depth-image features can further improve accuracy on top of UADD, at the cost of interpretability; in practice, the best cross-dataset performance is achieved by pairing AugLift (or AugLiftV2) with image-feature fusion.


==> sec/6_conclusion_tmp.tex <==
% \section{Conclusion}
% \label{sec:conclusion}

% We introduced AugLift, a simple, modular input representation that enriches the standard 2D keypoint input for lifting-based 3D HPE with synergistic confidence and depth cues. Our extensive experiments show that this approach is a powerful mechanism for improving generalization without sacrificing in-domain accuracy. Across three training datasets and four distinct lifting architectures, AugLift consistently reduces out-of-distribution MPJPE by an average of 10.1\% while also improving in-distribution performance by 4.0\%. 
% % The gains are largest for short-sequence models, indicating that rich spatial cues can effectively offset temporal context. In addition, AugLift does not require a depth sensor or external data collection.

% This work opens several avenues for future research. While our initial analysis shows that inference latency is manageable, a more thorough study is warranted, and future work could explore distilling the depth model's knowledge into a lightweight, unified architecture to enable real-time performance. We briefly discuss the inference time requirements in Appendix Section \ref{sec:inference_constraints}. Furthermore, our findings on the brittleness of motion priors suggest a need for deeper investigation into the role of temporal context; future research could explore how much the reliance on motion can be reduced when stronger per-frame inputs like AugLift's are available. 
% % Finally, as this is the first work to demonstrate the power of this specific combination of cues, significant research remains in tuning AugLift's hyperparameters and exploring other pre-trained priors to further unlock the potential of this approach.

\vspace{-5pt}
\section{Conclusion}
\label{sec:conclusion}

We introduced AugLift, a simple, modular augmentation of standard 2D--3D lifting that enriches each 2D keypoint with an Uncertainty-Aware Depth Descriptor combining monocular depth statistics and detector confidence.
Across four datasets and four lifting architectures in the realistic detection setting, AugLift consistently improves cross-dataset (OOD) performance by an average of 10.1\% while also improving in-distribution (ID) performance by 4.0\%, without requiring any new sensors, data collection, or changes to the core lifting architectures.
Our post-hoc analysis shows that these gains concentrate on hard cases—occluded joints and novel poses.
% where confidence-aware depth cues are most effective. 
We also find that AugLift complements dense image features, and that a learned depth-feature variant (AugLiftV2) offers additional improvements at the cost of interpretability.
% Our post-hoc analysis shows that these gains concentrate on the hard cases—occluded joints and novel pose configurations—where confidence-aware depth cues are most effective.
% We further demonstrate that AugLift is complementary to dense image features, and that a learned depth-feature variant (AugLiftV2) can yield additional improvements at the cost of interpretability.

% This work opens several avenues for future research. 
While our initial measurements suggest inference latency is manageable, a fuller efficiency analysis is warranted; one direction is distilling the depth estimator into a lighter-weight, unified architecture for real-time use (see Appendix F). Our findings on the brittleness of motion priors further highlight the need to understand how much temporal context remains necessary when strong per-frame cues like UADD are available. Finally, AugLift-style descriptors could be extended to multi-person scenes, other 3D prediction tasks, and settings with weaker or self-supervised depth signals.

% This work opens several avenues for future research.
% While our initial measurements indicate that inference latency is manageable, a more thorough study of efficiency is warranted; one promising direction is to distill the depth estimator into a lighter-weight, unified architecture to enable real-time deployment (see Appendix F).
% Our findings on the brittleness of motion priors also suggest the need for a deeper understanding of temporal context, including how far reliance on motion can be reduced when strong per-frame cues like UADD are available.
% Finally, it will be interesting to explore extending AugLift-style descriptors to multi-person scenes, other 3D prediction tasks, and settings with weaker or self-supervised depth signals.



==> sec/6_poseaug_dg_tmp.tex <==
%==============================================================================
\section{AugLift with Differentiable Domain Generalization}
\label{sec:poseaug_dg}
%==============================================================================

We now demonstrate that AugLift can be combined with a differentiable domain generalization method---PoseAug---to achieve state-of-the-art results for cross-dataset 3D pose estimation in the ground-truth 2D detection setting.

\subsection{Method}
\label{ssec:poseaug_method}

\paragraph{Integration with PoseAug.}
For these experiments we use the XYD input representation (omitting the confidence channel, which is not critical in the GT 2D setting). We integrate PoseAug's differentiable augmentation framework, which applies rotation-translation (RT), bone angle (BA), and bone length (BL) transformations in 3D pose space before projection to 2D. To generate geometrically consistent depth for augmented poses, we develop an analytical BA/BL$\to$SMPL mapping that converts augmented skeletons into SMPL body model parameters, achieving sub-millimeter accuracy ($<$0.2mm MPJPE) with 1,500$\times$ speedup over iterative optimization. Full details of the PoseAug framework and SMPL mapping are provided in Appendix~\ref{sec:poseaug_smpl_details}.

\paragraph{Depth extraction pipeline.}
The resulting SMPL meshes are rendered at 128$\times$128 resolution via differentiable rasterization, then processed by Depth Anything V2 to extract monocular depth maps. Per-joint depth values are sampled at 2D keypoint pixel locations via grid sampling, forming the D channel concatenated with detected 2D keypoints (X, Y) as the final XYD input to the lifting network. This pipeline enables live generation of viewpoint- and anatomy-augmented depth signals during training, where the depth channel adapts coherently to each augmented pose rather than using fixed pre-computed depth from original viewpoints.

\paragraph{Depth-based 2D rescaling (dscale2d).}
The raw XYD representation provides depth as an independent channel but does not account for the relationship between subject distance and 2D projection scale. Subjects closer to the camera appear larger in 2D, creating a systematic domain gap: 3DPW subjects are on average ${\sim}30\%$ closer than Human3.6M training data (mean root depth 3.6m vs.\ 5.15m). We address this with depth-based 2D rescaling, which scales the 2D keypoint coordinates by the ratio of estimated root depth to a reference depth: $(x', y') = (x, y) \cdot d_{\text{root}} / d_{\text{ref}}$. This normalizes 2D scale variations caused by distance differences, allowing the lifting network to see distance-invariant 2D patterns. The reference depth $d_{\text{ref}}$ is a hyperparameter; we find $d_{\text{ref}} = 4.5$m optimal via sweep over the range 3.5--6.0m.

\begin{figure}[tb]
\centering
\includegraphics[trim=0 0 350pt 0, clip, width=0.95\textwidth]{arXiv-2508.07112v3/figures/example_00.png}
\caption{\textbf{AugLift pipeline illustration: PoseAug bone angle (BA) augmentation with SMPL integration.} Left to right: (1) Original RGB frame from Human3.6M, (2) SMPL mesh reconstructed from the original pose, (3) SMPL mesh after analytical BA augmentation (perturbed joint angles mapped via SVD/Rodrigues IK), (4) Depth Anything V2 depth map extracted from the BA-augmented render. The analytical BA$\to$SMPL mapping achieves sub-millimeter accuracy (0.17mm mean MPJPE) while enabling live depth generation for augmented poses. Grid sampling extracts depth values at 2D keypoint locations to form the D channel, which is concatenated with 2D joint coordinates (XY) as input to the 3D pose lifting network.}
\label{fig:poseaug_pipeline}
\end{figure}

\subsection{Experiments}
\label{ssec:poseaug_experiments}

Our experimental setup involves several key design choices: (1)~an analytical BA/BL$\to$SMPL mapping achieving sub-millimeter accuracy with 1,500$\times$ speedup over iterative optimization; (2)~integration of live SMPL rendering and depth extraction into PoseAug's augmentation loop; (3)~comprehensive reproduction of DAF-DG showing its published SOTA is unreproducible from official code; and (4)~a format-decoupled 3DPW evaluation protocol that separates true domain gap from skeleton format artifacts.

\begin{table}[tb]
\centering
\caption{\textbf{Cross-dataset evaluation (MPJPE~$\downarrow$, mm).} All methods train on Human3.6M only. Published results from respective papers. $^\dagger$DAF-DG result unreproducible from official code; our best reproduction achieves 80.5mm. Independent users report the same issue {\color{blue}[TODO: cite]}. AugLift+ uses XYD input with depth-based 2D rescaling ($d_{\text{ref}} = 4.5$m).}
\label{tab:poseaug_crossdataset}
\small
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{3DHP} & \textbf{3DPW} \\
\midrule
VPose (1-frame)                     & 102.3 & 125.7 \\
PoseGU                              & 75.0  & ---   \\
PoseAug                             & 73.0  & 119.0 \\
DH-AUG                              & 71.2  & 112.8 \\
CEE-Net                             & 69.7  & ---   \\
DAF-DG$^\dagger$                    & \sout{63.1}  & \sout{106.6} \\
\hdashline
AugLift+ (XYD)                      & 62.9        & 104.3 \\
AugLift+ (XYD+dscale2d)             & \textbf{62.4} & \textbf{92.6} \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Results.}
\label{ssec:dafdg_comparison}

As shown in Table~\ref{tab:poseaug_crossdataset}, AugLift+---simply AugLift combined with PoseAug---achieves state-of-the-art cross-dataset performance on both benchmarks. On 3DHP test, our XYD+dscale2d model achieves 62.4mm MPJPE, a 14.5\% relative improvement over PoseAug (73.0mm) and 8.8mm below the next reproducible published result (DH-AUG, 71.2mm). On 3DPW, we achieve 92.6mm, a 22.2\% relative improvement over PoseAug (119.0mm) and 20.2mm below DH-AUG (112.8mm). The previously claimed SOTA (DAF-DG: 63.1mm 3DHP, 106.6mm 3DPW) is unreproducible from official code---our best reproduction achieves 80.5mm, and independent users report the same issue {\color{blue}[TODO: cite]}.

\subsubsection{Key Findings.}

\begin{enumerate}[nosep,leftmargin=*]
    \item \textbf{Depth augmentation helps}: Adding monocular depth and depth-based 2D rescaling reduces MPJPE from 74.0mm (PoseAug) to 62.4mm on 3DHP (15.7\% reduction) and from 119.0mm to 92.6mm on 3DPW (22.2\% reduction).
    \item \textbf{Incremental gains}: XYD without rescaling already outperforms all published methods (62.9mm 3DHP); adding dscale2d provides a further 0.5mm improvement on 3DHP and 11.7mm on 3DPW, confirming that both depth and scale contribute.
    \item \textbf{Cross-dataset generalization}: The combination of depth-augmented input and PoseAug's differentiable augmentation framework improves robustness to domain shift across both benchmarks, with especially large gains on 3DPW where the distance domain gap is most pronounced.
\end{enumerate}

